ViViDex: Learning Vision-based Dexterous Manipulation from Human Videos

In this work, we aim to learn a unified vision-based policy for multi-fingered robot hands to manipulate a variety of objects in diverse poses. Though prior work has shown benefits of using human videos for policy learning, performance gains have been limited by the noise in estimated trajectories. Moreover, reliance on privileged object information such as ground-truth object states further limits the applicability in realistic scenarios. To address these limitations, we propose a new framework ViViDex to improve vision-based policy learning from human videos. It first uses reinforcement learning with trajectory guided rewards to train state-based policies for each video, obtaining both visually natural and physically plausible trajectories from the video. We then rollout successful episodes from state-based policies and train a unified visual policy without using any privileged information. We propose coordinate transformation to further enhance the visual point cloud representation, and compare behavior cloning and diffusion policy for the visual policy training. Experiments both in simulation and on the real robot demonstrate that ViViDex outperforms state-of-the-art approaches on three dexterous manipulation tasks.

==> _constants.tex <==
\def\cvprPaperID{9893}
\def\confName{CVPR}
\def\confYear{2023}

\def\paperTitle{Paper Title}

\def\authorBlock{
    Author 1\thanks{Equal contribution} \qquad
    Author 2\footnotemark[1] \qquad
    Author 3 \\
    Institute \\
    {\tt\small \{email, addresses\}@inst.edu}
}

\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> tabs/sota_visual.tex <==
% \usepackage{multirow}
% \begin{table}[!ht]
% \centering
% \caption{Comparison with state-of-the-art methods on the \emph{relocate} task for the visual policy under ${\rm S@10}$. A single visual policy model is expected to solve all these 15 settings with different objects and initial object poses.}
% \setlength{\tabcolsep}{4pt}
% \renewcommand\arraystretch{1.2}
% \begin{tabular}{lcccccc}
% \toprule
% Methods & M. Bottle & TS. Can & S. Box & L. Clamp & Mug & Avg. \\ \midrule
% DexMV~\cite{qin2022dexmv} &  &  &  &  &  &  \\
% ILAD~\cite{wu2023learning} &  &  &  &  &  &  \\
% Ours &\textbf{1.00}&\textbf{1.00}&\textbf{1.00}&0.99&0.99&\textbf{1.00} \\ \bottomrule
% \end{tabular}
% \label{tab:visual_sota_relocate}
% \end{table}

\begin{table}[!ht]
\centering
\caption{Comparison with variants of our visual policy that use assumptions in previous methods under ${\rm S@10}$.}
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{ccc|ccccc|c|c}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Obj.\\ States\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Comp.\\ PCs\end{tabular}} & \multicolumn{5}{c|}{Relocate} & \multirow{2}{*}{Pour} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Place\\ inside\end{tabular}} \\
 &  &  & MB. & TC. & SB. & LC. & Mug &  &  \\ \midrule
DexMV~\cite{qin2022dexmv}&\checkmark&$\times$&  &  &  &  &  &  &  \\
ILAD~\cite{wu2023learning}&\checkmark&\checkmark&  &  &  &  &  &  &  \\
Ours&$\times$&$\times$&0.94&1.00&0.98&0.98&0.96&  &  \\ \bottomrule
\end{tabular}
\label{tab:visual_sota}
\end{table}

==> tabs/traj_aug.tex <==
\begin{table}[]
\centering
\caption{The performance of our state-based policy using different types of reference trajectory augmentation.}
\setlength{\tabcolsep}{3pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{3}{c}{Reference trajectory augmentation} & \multirow{2}{*}{${\rm S@10}\uparrow$} & \multirow{2}{*}{${\rm S@5}\uparrow$} & \multirow{2}{*}{${\rm S@3}\uparrow$} \\
 & initial pos. & initial rot. & target pos. &   &  &  \\ \hline
A1&$\times$&$\times$&$\times$& 0.00&0.00&0.00\\
A2&$\times$&$\times$&\checkmark&0.02&0.00&0.00\\
A3&\checkmark&$\times$&\checkmark&  &  &  \\
A4&\checkmark&\checkmark&\checkmark&\textbf{1.00}&\textbf{1.00}&\textbf{1.00}\\
\bottomrule
\end{tabular}
\label{tab:traj_aug}
\end{table}

==> tabs/visual_multi_video.tex <==
\begin{table}[t]
\centering
\caption{
Performance of separate policies for each object on the \emph{relocate} task. The initial configurations in testing are derived from all three rows in Figure~\ref{fig:object_pose}. We compare our visual policies using different number of training videos.
% Ablation studies of policies using different number of training videos. We train the policy for each object separately and test the policy under three different initial object configurations for each object as shown in Figure~\ref{fig:object_pose}. 
``Mb.", ``Tc.", ``Sb." and ``Lc." denote \emph{mustard bottle}, \emph{tomato can}, \emph{sugar box} and \emph{large clamp} respectively.
}
\label{tab:visual_multi_video}
% \scriptsize
\scriptsize
\setlength{\tabcolsep}{0.9pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{cc|cc|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Num.\\videos\end{tabular}} & \multicolumn{2}{c|}{Mb.} & \multicolumn{2}{c|}{Tc.} & \multicolumn{2}{c|}{Sb.} & \multicolumn{2}{c|}{Lc.} & \multicolumn{2}{c|}{Mug} & \multicolumn{2}{c}{Avg.} \\
 &  &${\rm SR_{10}}$&${\rm SR_{3}}$&${\rm SR_{10}}$&${\rm SR_{3}}$&${\rm SR_{10}}$&${\rm SR_{3}}$&${\rm SR_{10}}$&${\rm SR_{3}}$&${\rm SR_{10}}$&${\rm SR_{3}}$&${\rm SR_{10}}$&${\rm SR_{3}}$ \\ \midrule
BC&1&0.33&0.33&0.33&0.33&0.33&0.33&0.34&0.32&0.37&0.33&0.34&0.33\\
BC & 2 &0.66&0.64&0.66&0.66&0.66&0.65&0.65&0.50&0.70&0.67&0.67&0.62 \\
BC & 3 &0.96&0.92&0.98&0.97&0.98&0.97&0.95&0.90&1.00&0.97&0.97&0.95 \\ 
Diff & 3 &0.99&0.98&1.00&1.00&1.00&1.00&0.98&0.94&1.00&1.00&1.00&0.98 \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\end{table}
